X$^3$KD: Knowledge Distillation Across Modalities, Tasks and Stages for Multi-Camera 3D Object Detection

Recent advances in 3D object detection (3DOD) have obtained remarkably strong results for LiDAR-based models. In contrast, surround-view 3DOD models based on multiple camera images underperform due to the necessary view transformation of features from perspective view (PV) to a 3D world representation which is ambiguous due to missing depth information. This paper introduces X$^3$KD, a comprehensive knowledge distillation framework across different modalities, tasks, and stages for multi-camera 3DOD. Specifically, we propose cross-task distillation from an instance segmentation teacher (X-IS) in the PV feature extraction stage providing supervision without ambiguous error backpropagation through the view transformation. After the transformation, we apply cross-modal feature distillation (X-FD) and adversarial training (X-AT) to improve the 3D world representation of multi-camera features through the information contained in a LiDAR-based 3DOD teacher. Finally, we also employ this teacher for cross-modal output distillation (X-OD), providing dense supervision at the prediction stage. We perform extensive ablations of knowledge distillation at different stages of multi-camera 3DOD. Our final X$^3$KD model outperforms previous state-of-the-art approaches on the nuScenes and Waymo datasets and generalizes to RADAR-based 3DOD. Qualitative results video at https://youtu.be/1do9DPFmr38.

==> figs/qualitative_sup/qualitative.tex <==
\begin{figure*}
    \captionsetup{font=small, belowskip=-12pt}
    \centering
    \includegraphics[width=0.96\linewidth]{figs/qualitative_sup/qualitative_sup1.jpg}
    \includegraphics[width=0.96\linewidth]{figs/qualitative_sup/qualitative_sup2.jpg}
    \includegraphics[width=0.96\linewidth]{figs/qualitative_sup/qualitative_sup4.jpg}
    \includegraphics[width=0.96\linewidth]{figs/qualitative_sup/qualitative_sup5.jpg}
    \includegraphics[width=0.96\linewidth]{figs/qualitative_sup/qualitative_sup3.jpg}
    \vspace{-10pt}
    \caption{\textbf{Qualitative results on nuScenes}: We show the multi-camera input (top) and bounding box visualizations (bottom). We compare ResNet-101-based X$^3$KD$_\text{all}$ to BEVDepth$^\dagger$ and the ground truth (GT) for a resolution of $640 \times 1600$. Best viewed on screen and in color.}
    \label{fig:qualitative-supp}
\end{figure*}


==> include/supp_qualitative.tex <==
\section{Qualitative Analysis}

\input{figs/qualitative_sup/qualitative.tex}

We provide additional qualitative examples for X$^3$KD in comparison to the baseline BEVDepth$^\dagger$ and the ground truth (GT) in Fig.~\ref{fig:qualitative-supp}. In the first example from the top, we observe that the orientation of trucks and trailers (red and green boxes) is not well predicted by the baseline BEVDepth$^\dagger$ and some objects are not detected at all. While the predictions of X$^3$KD are also not perfect, most objects are detected and the orientation of objects is better aligned, which is also apparent by comparing the X$^3$KD output to the GT. We attribute the better detection to the additional guidance from instance segmentation in PV, while a better orientation and prediction in bird's eye view (BEV) is likely due to guidance from the LiDAR-based 3DOD model. More examples of objects that are difficult to  detect are given in the second and third example. In the second example, the bicycle (pink box) is quite far away and appears rather small in the front camera image. Similarly, in the third example the truck (green box) and the car (blue box) appear small and the car is partially occluded. Guidance from instance segmentation in perspective view can help to detect these rather difficult examples. This improved detection behavior also generalizes to adverse weather conditions as can be seen in the fourth example. Again, a bicycle is detected by X$^3$KD but not by the baseline BEVDepth$^\dagger$. Finally, the fifth example provides additional evidence on how the guidance from the LiDAR-based 3DOD teacher improves the translation and orientation characteristics of the predicted bounding boxes. The barriers (light green boxes) in BEVDepth$^\dagger$ are oriented rather random, while there is a structurally meaningful orientation observable for X$^3$KD.


==> tables/supp_ablation_main_nuscenes.tex <==
\begin{table*}[t]
\captionsetup{font=small, belowskip=-14pt}
	\footnotesize
    \centering
    \setlength{\tabcolsep}{7.5pt}
    \def\arraystretch{0.97}%
    \begin{tabular}{l|ccccc|ccccc|cc}
        \toprule
        \textit{Model} & Pre. &
        X-OD & X-FD & X-AT & X-IS & 
        \cellcolor[HTML]{96bbce}\textit{mATE}$\downarrow$ & 
    	\cellcolor[HTML]{fb9a99}\textit{mASE}$\downarrow$ & 
     	\cellcolor[HTML]{fc4538}\textit{mAOE}$\downarrow$ & 
    	\cellcolor[HTML]{fdbf6f}\textit{mAVE}$\downarrow$ & 
    	\cellcolor[HTML]{ff7f00}\textit{mAAE}$\downarrow$ & 
    	\cellcolor[HTML]{ab9ac0}\textit{mAP}$\uparrow$ & 
    	\cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ \\
    	\midrule
        BEVDepth$^\dagger$ & \ch & \xm & \xm & \xm & \xm & 0.644 & 0.274 & 0.455 & 0.350 & 0.211 & 37.7 & 49.5 \\        
        X-OD & \ch & \ch & \xm & \xm & \xm & 0.634 & 0.276 & \underline{0.451} & 0.343 & \underline{0.204} & 38.1 & 50.0 \\
        X-FD & \ch & \xm & \ch & \xm & \xm & \underline{0.626} & \underline{0.270} & 0.475 & \textbf{0.333} & 0.209 & 38.2 & 50.0 \\
        X-AT & \ch & \xm & \xm & \ch & \xm & 0.654 & 0.273 & \textbf{0.439} & \underline{0.337} & 0.207 & 37.9 & 49.8 \\
        \rowcolor{gray85} X-IS & \ch & \xm & \xm & \xm & \ch & 0.635 & 0.273 & 0.462 & 0.350 & \underline{0.204} & \underline{38.7} & \underline{50.1} \\
        \rowcolor{gray8} \textbf{X$^{3}$KD}$_{\mathrm{all}}$ & \ch & \ch & \ch & \ch & \ch & \textbf{0.615} & \textbf{0.269} & 0.471 & 0.345 & \textbf{0.203} & \textbf{39.0} & \textbf{50.5} \\
        \midrule
        LiDAR Teacher & \nap & \nap & \nap & \nap & \nap & 0.301 & 0.257 & 0.298 & 0.256 & 0.195 & 59.0 & 66.4 \\
        \bottomrule
    \end{tabular}
    \vspace{-6pt}
    \caption{\textbf{Ablation study of X$^{3}$KD on the nuScenes validation set}: We incrementally add our proposed cross-modal feature distillation (X-FD), adversarial training (X-AT) and output distillation (X-OD) as well as our cross-task instance segmentation distillation (X-IS). All X$^{3}$KD variants in the top part are solely based on multi-camera images during inference. \textbf{Backbone weights are initialized with weights pretrained for instance segmentation on nuImages (Pre.).} Best numbers in boldface, second best underlined.}
    \label{tab:supp-ablation-main}
\end{table*}

==> tables/supp_backbones.tex <==
\begin{table}[t]
    \captionsetup{font=small, belowskip=-11pt}
    \footnotesize
    \centering
    \setlength{\tabcolsep}{7.0pt}
    \begin{tabular}{l|cc|cc}
        \toprule
        \textit{Model} 
        &  \textit{Backbone} 
        & \textit{Resolution}
        & \cellcolor[HTML]{ab9ac0}\textit{mAP}$\uparrow$ 
        & \cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ \\
        \midrule
        BEVDepth$^\dagger$ & ResNet-50 & $256\times 704$ & 35.9 & 47.2 \\
        \rowcolor{gray8} \textbf{X$^3$KD} (Ours) & ResNet-50 & $256\times 704$ & \textbf{39.0} & \textbf{50.5} \\
        \midrule
        BEVDepth$^\dagger$ & ConvNeXt-T & $256\times 704$ & 38.3 & 50.8 \\
        \rowcolor{gray8} \textbf{X$^3$KD} (Ours) & ConvNeXt-T & $256\times 704$ & \textbf{39.7} & \textbf{51.9} \\
        \midrule
        BEVDepth$^\dagger$ & ResNet-101 & $640\times 1600$ & 42.8 & 53.6 \\
        \rowcolor{gray8} \textbf{X$^3$KD} (Ours) & ResNet-101 & $640\times 1600$ & \textbf{46.1} & \textbf{56.7} \\
        \bottomrule
    \end{tabular}\vspace{-5pt}
    \caption{\textbf{Ablation on varying backbones}: We show that X$^3$KD improves ResNet-based as well as ConvNeXt-based models on top of BEVDepth$^\dagger$ (re-implementation of~\cite{li2022bevdepth}).}
    \label{tab:supp-ablation-backbones}
\end{table}

==> tables/supp_hyperparameters.tex <==
\begin{table}[t]
    \captionsetup{font=small, belowskip=-6pt}
    \footnotesize
    \centering
    \setlength{\tabcolsep}{12.3pt}
    \begin{tabular}{l|cc|cc}
        \toprule
        \textit{Model} 
        &  Pre. 
        & $\lambda^{\text{X-AT}}$
        & \cellcolor[HTML]{ab9ac0}\textit{mAP}$\uparrow$ 
        & \cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ \\
        \midrule
        BEVDepth$^\dagger$ & \ch & $0$ & 37.7 & 49.5 \\
        & \ch & $1$ & 37.6 & 49.4 \\
        \rowcolor{gray85} X-AT & \ch & $10$ & \textbf{37.9} & \textbf{49.8} \\
        & \ch & $20$ & 37.8 & 49.7 \\
        \bottomrule
    \end{tabular}\vspace{-5pt}
    \caption{\textbf{Ablation on the X-AT loss weight}. We initialize all models with backbones pre-trained on nuImages (Pre.).}
    \label{tab:supp-ablation-x-at}
\end{table}

\begin{table}[t]
    \captionsetup{font=small, belowskip=-6pt}
    \footnotesize
    \centering
    \setlength{\tabcolsep}{12.3pt}
    \begin{tabular}{l|cc|cc}
        \toprule
        \textit{Model} 
        &  Pre. 
        & $\lambda^{\text{X-FD}}$
        & \cellcolor[HTML]{ab9ac0}\textit{mAP}$\uparrow$ 
        & \cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ \\
        \midrule
        BEVDepth$^\dagger$ & \ch & $0$ & 37.7 & 49.5 \\
        & \ch & $2$ & 37.8 & 49.6 \\
        \rowcolor{gray85} X-FD & \ch & $10$ & \textbf{38.2} & \textbf{50.0} \\
        & \ch & $25$ & 38.1 & 49.7 \\
        & \ch & $100$ & 37.3 & 48.8 \\
        \bottomrule
    \end{tabular}\vspace{-5pt}
    \caption{\textbf{Ablation on the X-FD loss weight}. We initialize all models with backbones pre-trained on nuImages (Pre.).}
    \label{tab:supp-ablation-x-fd}
\end{table}


==> tables/supp_hyperparameters2.tex <==
\begin{table}[t]
    \captionsetup{font=small, belowskip=-6pt}
    \footnotesize
    \centering
    \setlength{\tabcolsep}{11.3pt}
    \begin{tabular}{l|cc|cc}
        \toprule
        \textit{Model} 
        &  Pre. 
        & $\alpha^{\text{3D-bbox}}$
        & \cellcolor[HTML]{ab9ac0}\textit{mAP}$\uparrow$ 
        & \cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ \\
        \midrule
        BEVDepth$^\dagger$ & \ch & \nap & 37.7 & 49.5 \\
        & \ch & $0.8$ & 37.9 & 49.8 \\
        \rowcolor{gray85} X-OD & \ch & $0.6$ & \textbf{38.1} & \textbf{50.0} \\
        & \ch & $0.3$ & 38.0 & 49.9 \\
        \bottomrule
    \end{tabular}\vspace{-5pt}
    \caption{\textbf{Ablation on the X-OD ground truth selection threshold}. We initialize all models with backbones pre-trained on nuImages (Pre.).}
    \label{tab:supp-ablation-x-od}
\end{table}

\begin{table}[t]
    \captionsetup{font=small, belowskip=-6pt}
    \footnotesize
    \centering
    \setlength{\tabcolsep}{11.3pt}
    \begin{tabular}{l|cc|cc}
        \toprule
        \textit{Model} 
        &  Pre. 
        & $\alpha^{\text{2D-bbox}}$
        & \cellcolor[HTML]{ab9ac0}\textit{mAP}$\uparrow$ 
        & \cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ \\
        \midrule
        BEVDepth$^\dagger$ & \ch & $1.0$ & 37.7 & 49.5 \\
        & \ch & $0.8$ & 37.9 & 49.8 \\
        & \ch & $0.5$ & 38.0 & 50.0 \\
        \rowcolor{gray85} X-IS & \ch & $0.2$ & \textbf{38.7} & \textbf{50.1} \\
        & \ch & $0.1$ & 38.2 & 49.9 \\
        \bottomrule
    \end{tabular}\vspace{-5pt}
    \caption{\textbf{Ablation on the X-IS ground truth selection threshold}. We initialize all models with backbones pre-trained on nuImages (Pre.).}
    \label{tab:supp-ablation-x-is}
\end{table}


==> tables/supp_more_baselines.tex <==
\begin{table}[t]
    \captionsetup{font=small, belowskip=-8pt}
    \centering
    \footnotesize
    \def\arraystretch{0.95}%
    \setlength{\tabcolsep}{2.1pt}
    \setlength{\aboverulesep}{-0.3pt}
    \setlength{\belowrulesep}{1.0pt}
    \begin{tabular}{l|c|c|c|c}
        \toprule
        model & BEVDet & BEVDet + X$^3$KD & BEVDet4D & BEVDet4D + X$^3$KD \\
        \midrule
        \cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ & 37.9 & 41.3 & 45.7 & 49.1 \\
        \bottomrule
    \end{tabular}
    \vspace{-8pt}
    \caption{Combination of X$^3$KD with BEVDet and BEVDet4D.}
    \label{tab:transferability}
\end{table}

==> tables/supp_train_comp.tex <==
\begin{table}[t]
    \captionsetup{font=small, belowskip=-15pt}
    \centering
    \footnotesize
    \def\arraystretch{0.95}%
    \setlength{\tabcolsep}{2.4pt}
    \setlength{\aboverulesep}{-0.3pt}
    \setlength{\belowrulesep}{1.0pt}
    \begin{tabular}{l|c|cccc|c}
        \toprule
        model & BEVDepth & X-AT & X-FD & X-OD & X-IS & \textbf{X$^3$KD} \\
        \midrule
        training time & \SI{54}{h} & \SI{65}{h} & \SI{65}{h} & \SI{67}{h} & \SI{73}{h} & \SI{78}{h} \\
        GPU memory & \SI{39}{GB} & \SI{44}{GB} & \SI{44}{GB} & \SI{44}{GB} & \SI{48}{GB} & \SI{52}{GB} \\
        \midrule
        \cellcolor[HTML]{a5eb8d}\textit{NDS}$\uparrow$ & 47.2 & 48.1 & 48.5 & 48.7 & 50.1 & 50.5 \\
        \bottomrule
    \end{tabular}
    \vspace{-8pt}
    \caption{Training complexity/performance trade-off when training on 4 NVIDIA A100 GPUs with a batch size of 16 per GPU.}
    \label{tab:train-complexity}
\end{table}
